Causal functional calculus

We construct a new topology on the space of stopped paths and introduce a calculus for causal functionals on generic domains of this space. We propose a generic approach to pathwise integration without any assumption on the variation index of a path and obtain functional change of variable formulas which extend the results of \follmer\ (1981) and Cont \& Fourni\'e (2010) to a larger class of functionals, including \follmer's pathwise integrals. We show that a class of smooth functionals possess a pathwise analogue of the martingale property. For paths that possess finite quadratic variation, our approach extends F\"ollmer-Ito calculus and removes previous restriction on the time partition sequence. We introduce a foliation structure on this path space and show that harmonic functionals may be represented as pathwise integrals of closed 1-forms.

==> arbitrage.tex <==
A strategy is a pair $(\phi,\psi)$ of continuous function on $\Lambda$, where $\phi$ is $\R^{m}$-valued and $\psi$ is real valued. The value is $V:=\phi_{-}\cdot x+\psi_{-}$. A strategy is \emph{self-financing} if
\begin{itemize}
    \item [(i)] $\Delta\phi(t,x_t)\cdot x(t)+\Delta\psi(t,x_t) =0$,
    \item [(ii)] $\left(\phi(t+h,x_t)-\phi(t,x_t)\right)\cdot x(t)+\psi(t+h,x_t)-\psi(t,x_t)=0$.
\end{itemize}

\begin{Eg}[self-financing strategy]\noindent\\
If $(\phi,\psi)$ is self-financing, then $\phi$ is integrable and\begin{eqnarray*}
\int_0^{t}\phi dx=V(t,x_t)-V(0,x_0)
\end{eqnarray*}
\end{Eg}

\begin{proof}
We first obtain $\nabla_{x}V=\phi_{-}$, which is left-continuous and strictly causal. (i) implies that $V=\phi\cdot x+\psi$ which is continuous and by (ii), $\D V$ vanishes, hence $V\in \M$. The claim follows by an application of Cor.~\ref{cor:ftc}(ii).
\end{proof}
 
\begin{Rem}
Differentiability is not imposed on $V$ and $(\phi, \psi)$.
\end{Rem}


         
 
  We remark here that \emph{arbitrage} does not exist regardless what the variation order a collection of paths may possess. 

==> intro.tex <==
\section{Introduction}\label{sec:intro}

    
    For decades, \follmer's theory of pathwise integration \cite{HF} (1981) and its extensions may best be understood by one-form, that is if \begin{eqnarray*}\phi\in\{\nabla_{x}f|f\in C^{1,2}(\mathbb{R}^d)\},\end{eqnarray*}then $\int\phi dx$ is defined as (uncompensated) limit of left Riemann sums i.e. \begin{eqnarray}
    \int_{0}^{t}\phi dx:=\lim_n\sum_{\pi_n\ni t_i\leq t}\phi(t_i,x(t_i))\left(x(t_{i+1})-x(t_{i})\right),\label{eq:intro.integral}
    \end{eqnarray}along a vanishing sequence of time partitions $\pi_n$ of which $x$ admits finite quadratic variation. This integration approach has been extended in multiple directions (under the uniform topology). Most notably, the extension for $C^{1,p}$ functionals driven by continuous paths of $p$th order variation \cite{CP2019}. 
    
    The notion of a pathwise integral as  limit of left Riemann sums is fundamental in mathematical finance due to its interpretation as the gain of a sequence of bets $\phi(t_i,x(t_i))$ placed against price movements $x(t_{i+1})-x(t_{i})$. This interpretation of (\ref{eq:intro.integral}) would be compromised \eqref{eq:intro.integral} is replaced by a  compensated Riemann sum as in rough integration theory \cite{CP2019,FrizHairer}. This would in general, be the case if one were to extend the results of \cite{CP2019} to \cadlag paths with higher order variation. 
    
    An important question remains however: How do we characterise the class of uncompensated pathwise integrals, which are the most relevant in applications, for paths of higher order variation or more generally on a generic path space?
    
\subsection{The generic approach}
    
    Looking at (\ref{eq:intro.integral}) from a different perspective, we observe that \follmer's integral\begin{eqnarray*}
     F(t,x):=\int_{0}^{t}\phi(s,x(s-))dx(s)
    \end{eqnarray*}is a \emph{functional}, well defined everywhere at which $x$ admits finite quadratic variation. Further, there exists a bespoke topology defined on a suitable domain which makes $F$ a continuous functional. In particular, \follmer's integral possesses the following differential characteristics (unbeknown to the existing literature): \begin{eqnarray}
    \D_t F=\nabla^{(p)}_{x}F=0\label{eq:intro.char}
    \end{eqnarray}for all $p\geq 2$. The meaning is clear, the bet $\nabla_{x}F(t,x)=\phi(t,x(t-))$ placed, is interpreted here as a "prevision" and is therefore "blind" to a perturbation of future price movement.
    
    In fact, all continuous functionals that satisfy (\ref{eq:intro.char}) are limits of left Riemann sums as well as canonical solutions (not necessarily continuous in the uniform topology) to the path-dependent heat equations \S\ref{sec:ftc}. This class of functional is called $\M$. The most crucial observation is that such a characterisation can be extended to other generic domains that include, but not limited to, paths of $p$th order variation.
    
    In order to demonstrate that all (uncompensated) left Riemann sums that may possibly be characterised by the one-form approach (i.e. associated with a $p$th order change of variable formula for $p\geq 2$) are in class $\M$, we deliberately start with an explicit definition of a pathwise integral on a generic domain, \emph{unassociated} with any change of variable formula and shows that it belongs to class $\M_0$ (i.e. $\M$ mod initial value) and vice versa. In doing so, we also recover the corresponding analogues of the classical fundamental theorem of calculus I \& II, which facilitates the evaluation of a pathwise integral. Most importantly, we are able to show that this generic notion of a pathwise integral is exactly equivalent to that of the value functional of a self-financing portfolio (mod initial capital) in mathematical finance. 

    Finally, since the differentials of a functional is independent of the variation order of a path, if one were able to characterise pathwise integral in terms of its differentials, then one can extend the notion of a pathwise integral to generic domains, by using only these differentials. Most importantly, this will lead to a fresh theory of path-dependent equations whose smooth solutions are not necessarily continuous in the uniform topology. 

\subsection{Relation with previous work}

{\bf You cannot avoid a discussion of relation with literature
This is one reason it was rejected previously
If people do not understand the link with what they know, they reject}

can we probably remove this section?or just discuss CF 2010? I worry it will be subject to lengthy multiple rounds of reviews or outright rejections by rough path theorists?
\cite{chevyrev2019}

Our aim is not to generalise an existing rich theory for irregular paths e.g. Lyon (1998), Friz \& Hairer (2014) but to introduce a bespoke and yet versatile calculus for causal random system in general and mathematical finance in particular, in order to solve problems practically.

\subsection{Outline}
		
		In this article, we introduce functional calculus based on a new topology. We extend the notion of pathwise integral to \closed{} domains, give existence condition of pathwise integral and obtain a general change of variable formula without any assumption on the variation index of paths. We show that pathwise integral belongs to class $\M$, a subclass of continuous and infinitely differentiable functionals. Using class $\M$ as \emph{primitives} (i.e. anti-derivative) and an analogue of the Fundamental theorem of calculus, we relate class $\M$ functional to the notion of a \emph{martingale}.
		
		We then apply our functional calculus to treat paths with finite quadratic variation. We obtain \ito's formula and an analytic analogue of \ito's isometry in the spirit of the pathwise BDG inequality of \cite{PS}, a formula of which, one may resort in order to extend the pathwise integral under (possibly a collection of) positive linear functional(s). In addition, we show that class $\M$ are canonical solutions to the path-dependent heat equations.
		
	
	The layout of this article is as follows. We introduce our notations in Preliminaries. In section~\ref{sec:qv}, we prove a new limit theorem which allows us to treat functionals that involve quadratic variation. In section~\ref{sec:pi}, we introduce a new topology on path spaces, relate it with other well-known topologies and give examples of continuous functionals. In section~\ref{sec:c1k}, we introduce functional calculus and smooth functionals, the class $C^{1,2}$, $\X$ and $\M$. In section~\ref{sec:ito}, we extend the notion of pathwise integral and prove change of variable formulas. In the final section~\ref{sec:ftc}, we obtain an analytic analogue of \ito's isometries and discuss the relation of class $\M$ to path-dependent equations.   
	

